Explaining how your AI system is fair

To implement fair machine learning in a sustainable way, choosing the right fairness objective is key. Since fairness is a concept of justice which comes in various, sometimes conflicting definitions, this is not a trivial task though. The most appropriate fairness definition for an artificial intelligence (AI) system is a matter of ethical standards and legal requirements, and the right choice depends on the particular use case and its context. In this position paper, we propose to use a decision tree as means to explain and justify the implemented kind of fairness to the end users. Such a structure would first of all support AI practitioners in mapping ethical principles to fairness definitions for a concrete application and therefore make the selection a straightforward and transparent process. However, this approach would also help document the reasoning behind the decision making. Due to the general complexity of the topic of fairness in AI, we argue that specifying "fairness" for a given use case is the best way forward to maintain confidence in AI systems. In this case, this could be achieved by sharing the reasons and principles expressed during the decision making process with the broader audience.

==> study-url.tex <==
\href{https://axa-rev-research.github.io/drawio/src/main/webapp/?chrome=0&grid=0&toolbar=0&p=props&title=Sample%20Study#R7V1Zl9s2lv41Ou08lA5JiZT0WC67nExncdvuSTwvPhAFSUhRpMJFVZVfP8DFQhCEKEpFbU5l5rRLXEAsF3e%2FH3qDu9XThxStl78kMxz1PGf21Bu863me7458%2Bg%2B78syvDLyRw68sUjLj19zywmfyNxYX5WMFmeGs8mCeJFFO1uKieC5M4hiHeeVBlKbJY%2FXdeRJVv7pGC1y78DlEUf3q72SWL8XVwHHKGz9isliKT9MOiTsrJJ8WF7IlmiWP2qXB%2B97gLk2SnP%2B1errDEZs%2BOTH8vfstd1XPUhznbV747b%2FTgfvvX2ZDMp94G%2F%2F29r9%2F%2FO%2BNJxYoy5%2FlkPGMzoD4maT5MlkkMYrel1ffpkkRzzBr1qG%2Fymd%2BTpI1vejSi3%2FiPH8Wy4mKPKGXlvkqEnfnSZyLmy77XR%2BKGF2WFGko%2BvU%2BmP32IV3%2BPb%2F9H%2FT07fH91%2FC%2F728CQRMoXeC8YZwT%2Fhwbm%2FYBMVEfcLLCefpMH0hxhHKyqa4%2BEkS0UM%2BpVz8mhHbZcwTF33jBZNJ3nIn6b8ybEPR%2F444Dp9ooH6Jop1w%2B%2BofWsfISLOo%2BCyxmaIOiQozqK91QtkX%2FGU3p9q0sFIrIIqZ%2Fh3RhcEovbHCaE7o9bsWNFZnNOE3gjPyNptAeo4o1GxAM0X%2Fb89%2B1WvRGCmVfxk%2BVdRGbXny1sq0qiyoXx%2BkPncCtLIj49dJlrzY6rL6fzOcZPsriuq51IY%2B8e%2Bl6pc9%2FsPf7vvz5VTQHP949VX49y19PJP9D%2B%2Ftr2QT9Vb7Efsh3uuMUXktOMToKp7hNU%2FSsPSC2RwMjGQ1HJutwHYOIeKvbaDKYDIwWguHRmM9%2F1rejR8f5CU9%2FX%2F46m3y8%2FW309kYO4WqZj9xgnTCf0djxqwsy7IT7DKqtdsB9kumfTJnynIivyjt4nXcVZUlM4oW8GEQ5WzX214L99Uk9IG7Rpsu78uJaXvgcEroCZE5CRkvxjC5vTpI4YwRSLBY4y4F80mdo0VmnyRRNSURywuiI6nMp0y7JfI5hJemw6bZlymRSrDNQFvlS5SmCAd0lGzK7cSd9rXvrsnfeTo471NZBbIHr4r7upXBf63PDU%2BlpXmBqZsHQaGYLc7Q0NtjdGB%2F5AZyW%2FhTbcR%2FFQCpNJeP9Nbkmvjvsiu86fWcyGHSj5Y0mJ1PsnNr6SYY1raxh8FfB7EeY55sMJvqWPuC66yfObsV9yeLe%2F1Ug4Fk4opNIOS1fDZI%2FawxxWmWIGsWU3Ist5uOS5PjzGsHOf0zR2rDySBTdJRFl0ezdwdxn%2F0evZ3maPGDtTgD%2FiVFo1%2Fl%2F%2B%2FChGr1sl8feZOwYm9b1BKE8aqa%2BVJmWmpU%2FcLbTToUUmkWq3JJdC9Wf2KrmSxCElNzZr4xuZrrMTBomc%2BadwEzUgrOGoEWcZHSDM3m5TiISctlKVzdcsktFmhWsLSxoJ8VruvHp1CNBQDPWbJyA%2BF2vo%2BeDhevo7ML1ABPlUIFsErXyD7GbfxartRxrnMRscNkDzsOluH%2B4JJZetF2S2GspiUv9duC6QTeMlrJtU6COzGbaS%2Bd6Y8GonXTe32objIfGtyaOa7CFJqvN6NchEuYghcE7jyfhAJ20q%2B12%2BA4a1HfQCT0JNlfByGv2OY5O7HP0atrLxzRZUwIhjDyuSA%2FdqlccYv%2Bb5v9RfI%2FjSV%2Bqu8dXU6W%2BdF0W8Hn8j225hlT9j882xiNTVg1bMor95eLENZVt%2BS2rXOyMQKUdWXIiaQHFxWqK02tyRsrd1oVR7Pov9D3KdRwP%2B0Ew0f47Fe8Z1gNbH1Mckgxskleu1I4rTepcyfpcW11GC7WNBgcJuP15y9g14hyTyV6BEtons4GWfNBmAHhGW2PTWbDF1ijbug7P%2FRfwL%2FDvscWl21U53Ncp3nB3PInn4GcqwLmAk3XEnpynyYpRJ30Ozbhnn7srZiSjvcB9%2BidzY81RlGHwSmREfES4K4juoaAct4gYjdDP0f%2BhDD5FcU74WBzUY84bFOXLZ%2BhDmoHTAlqgfDMjM5zSjS%2B6PsWqMxHOMsziC3hDInh4xbaYenRFskx8Iq4PVXzmcSkjECQusJqhnPYwW5HcNnI6symeJym9fMdagHle52TFdryMeVBWh6LoUE%2FL8GI8Lddl%2BrVll%2BO92aXMlHqxVufuZEDtmZkzPCsz2%2BXJsMac%2Fbpe8An2yhVpeipu3oXZ6Q7GQWUVO7I7B56t1U4VP3tSwVUZnQfxHitRDEYtmY%2Ffkvm0JoAtIY2Wy1U3wT4XYYgxW46L3JKNVNfJlgwGMpTYcSaIp5w%2FRsMn2JbXk0n6su0VXNb2qou7e0Si69pbXaZ4jv2Jsbc6kndDvx9UU%2FKOIfIaaVNbZL6SzPSIExmINRa8url2BeuPEWJ3a6EIfyS0Bj3E7llC7GaadHcbxqlN1Bn41KHqxOH8TY779Pxtm3XhSx%2Bkoo7BYFxt5uCsqZa04H0HzFOmCnWimARulXkq59ELY1QTk3fK%2FILjKyb%2B5BI2%2FAk2buc1Li%2Fis0E9he0a9X5JPR1lgAcvdPPIOrrThVnqyyhVjzBJU5lEeHGqx9Cpuidu3KFvye7rSPU4ndv9d%2BYCfkRx6Tnm3u%2Be7r9%2BBkcz%2BInjRHiRSb4UP500Afc7dyQTtrXWKeZK5KEOZV%2Bn%2FatJ3TupVtbkKN7J213vVFqZW%2FMgtKxYtAXWJoaG53vt%2FMcHJN55RoKBLLQ8ML%2FgoCw6XzKqklneRSjLFGO4SLnXsKE7knuOZ7igbxR3fBG1yjROxeM9av8HpxKNvncOxfI6A2et%2BdzgVHzOc0b9ydB1R8Fw5PjjcWdRM3di5gDLws0jmLV2wpS%2Bak31DiGefD3sR1rmnVR9u6a7vavUS5P%2FnIr1BFcVAztv6aFUnXZmXgYn07GUiaF0rJbcpjP6Gdc4xH0t1%2BZqmEXQYWKkNxmbhmMnvKLKKUaU%2FEcvZxanzvZKSfbQkxVkJAuZbstqt2UhWLZMimgmrVBZL4bCNAEdGJIwKhXah5qbwdWWYddMzgPM1lPwwpNlodcqpgadVascZMMFtoAqZ40xXiCRhqiqcdMK5e1bjtvz6P8718x6OyvUZgWEVc7bkZI2GvcN63N8Mu9pcJakCMVTFB%2F5qt25VFdYe97know3mbmUnum%2F2icx3ND5BsezCsf%2BYpA%2BPTx%2FmPwShfj%2B73cYY1tVXp2xnZ7xtGU0XeaIuGPfmsnx0mKYk9l%2FMsn1OnSe85a4uG0r72Q6wtmhvxxTJRoN9ytocYZG3s2oJd%2FqjD5l1FQrziprOELuE78aJUellHdgXw79YadVwGWRNzVdj8B%2B8l%2F%2FSBdforfBp2%2FZ9NH9PRs9%2BTLT4NXx3SX36Txt%2BzDuQ2WjyTxOxX3adCY4ntZkJXULEtOvpRl4wZysaeN2A6vlHMepXlW5vXEnnrJ2Yms0elWrWjO243iIDgBKNYM7%2B%2FKrIDDUrWAw6cvMhf0NvVp%2F%2FPFpw3%2BjuvJl9WBduetp1FmRHIOukvU9h3KvEzCn8avWtS9z2o3RdByty8ZljMzqm8B5CZcZ1pnWsVKrfFPQNzLYrsh9XFe8rplZyYBrJ37y6nJ4nehdXtUsHY37Eq6qU9ZmdU2eBXzuBdylzlyaIJ9On5Bv9%2F%2FW9tOZsNjrE99EFN0UBSos%2FBdXAXbg47WF7T8y4FX6%2BD1vfoazMCVriKvD%2FXoEX7zRKnz%2FLuHQIxDFx%2FGGpEm84ggtjwxthO37pOjxbPB41hPJ5DO8jpJn9SIDdy2D%2FWRF%2BTBcjnNyMyOswysSy9sKSZYNyfmy5M%2BuQPZkOYYEdA4DE6FHnqOe4kURyffL5HSADKS%2FFygmGZIYgvxooIjEeFsWgTEH99AifkIrAKG5U8OSTwJQTIrnMOEyUrvMc3bU0C1bXu9%2BnvYfyQNZ4xlBfdojeon9pv%2F8nJBvkra%2B9Tz%2FjtKbf%2Bt8i9A3hperrkwUcG751OSvgkRkqj2Ev1EC%2BDbHqxX9B%2Bfwa5nAL1R8yzCJ4RKDr8Ekyr7RFfO9EZrR%2BSdZnvL24b1vWZFu6DMRiilP0wLQOvuSV79N6WMPljD1e69H5fHk7o7yVtrF28nN%2FxHam3SF4ljefCeXUq0FKteCri0dZKpR4TRB6QzKFFg2CRIpHEn4AIsULlEMeSIRHQ9A7sDqZXTq8E3yGMMlAOSJOVoxIP%2Fcp3yUCvY%2FI3CAAP8E7DiM4ArTYHx555Hu1W2VD0ILkZx1uzzYmoyS0oWbFpSGdtXBzIgsp6F32ckHdW0DZWt%2BytWcPDHZ102tTOAZuqQ7kZnseq2MPNlKr5VRF%2FcQV7vSMqzS4CyB9MNVBK%2BlinCcYtsucIuDsXGcWIv6XeOdFxsGVkqo5%2Bf8KmqcpgXrXyUJ7WK1my7D2RN3fAJk2UCV8Hat%2B0hIzinKzNwqzoapQBOKREvdyGiRv79HoqP2Xk8C28GNtcIxVmIlzPm3pFWqSu%2FUHel1gzsbgJSTmlhOUm7RroXmwwDgPhcAa4dqHQkBaM6eXJkV7GQIefDNndKg8up76qwc9qGf5krxixNK8LinH7ZTnTwuYenDrNUZyhH%2FCH97iTZK7M5wSBUz9kLZeqVgcY5ISrW2DJ6dU41FTCe8TfWviBNIvoR5B8USUznPdF1Z05gLnLweVDGuYEq1VQp5z6lqG6suoCwrVlhMa4iKTJxlwKc9W5I1TFH%2BiLF2fAKbzh47LgHAYvlDiCvIFkLhd8SQBReKyAMuJ65x7Dl6wOXA6V5MYIFDKsa0AdMO5zDgRz3ZlurmlDRTIii2nHqxNLzws9SeeYJwD5AKGfWo5aO7kmC%2BmktULpo6UYk%2Bz6ZcJ6XoWTFf%2BoUlNEg7mRJ6rYRT5DRD2VukHT2SJiGfDVjYRLwsHoXFAU2P97Y88UliJpbnPunEyubqKwavbCybVOPlqqEwR9SRFoLGUcabImIL4Y0ghqRYLM2RlAdUwUceSSbMCgFOqdFRlYi3QE8mKVkw%2B0lDyKSUkNPL8qQO3cRS%2B7d5UylpSOIwKmZqmVec1oC6%2BZxmnOtkSUjgcyT%2Bs8gEUyDlUNagQN%2FJHcVZBbbyW6opRuUpXOsiK6eQKWYpJdcNifACpgAIbJsl1%2FNYtty2o05QTz%2FQpDzqpDTxjH7xAYPar3Yt%2Fxt6mhWMrspVoMYeZQycQFKNbKCuekkA0pSBDimDYpoKMyNk9ghQdhgWqeKi0uBwZFo906dbrCEKH%2BLkMQJt0cYggSbkjMBGgweZXZhloq3K7CyTRwwC6a5hO8le680wMxrmQ4of%2FWWcL2M40E0xjbDCqiRrUJRfxJKAkjUTr0UMB7wZJE4FSyTwV3XY2WT3JiiRaQVmQTO533EOkWSNxK0JVc4NCNfZBC9G4bJFdcN24%2BHl9uRpjMfhwLQC1BG35zAerSAeMrH8%2BtKwD7dAh3ULtBFb7EJgYyT6gI7Yz7Ck6RaMns9hzx2IGyNJrpPo9EjiYnWQJdjF6SCnqzv7ePeJETFVszgvnlE5HALU96dfWWXNG5DkCxzjHCTOijJnqgRHP%2FSU%2FgrMn7E%2BccooV7VBXmxICmjdXAPgDJ1%2FofaIwE9ZEtADERPniAvcL0VKJSpjFuwlslIWI%2BtVyslWV6Agw4nqkLCnmJdTUwQklMuM%2B%2Bv5mWrMzZkS4WoH93mhib9lsRL95mcftBA6VofEpFHoXHAaVKcs8qyAugc5Ri0Jipcd1%2BsSUGtcy6roxvXlj2pAuseo7bAv6JVFw9vuorPh5tpnWcrnc5%2BQ23LXdHoS%2BWTgdHRSY9BBzYFNm%2FigBGpagOBFG0QiPsT2bmCzFbvGsdW58Au14UjMjwJBqTxOJFokKVUGVqU7IE8R4RHJKZtnEWIuxTo4StYVW1R3rcGwVSSUX4MmhcrDvU38U8p%2BFb6NZ77%2BVD3KdV9bVqxZcF76Vco5YJ16h9c4FseuJJqPSni1sGqdGGbugh%2Bsglm77Il5NaJedXmpUSmlRnhTdNt9RbXBIsUsFUE5Afm6TrnbaUaydSHt6jmiqh8bwY%2B620J8Vfvemh9P2zP8Z6amlFVmcSUjZuzElYjjG8Y5AsVNvjklCL5%2Fm9WHmeF0g2ULKQZnSBmLZgrsCmkrtEpmOPoXd6FwXbInfagoyhL5Hst3yObQs17Fv8G2E6izatJhtZJYqZ%2B0%2BzNwgNRWWmCRle4xsblIBOdAi7gG5w5EzP3C3JDMgZiJ5zLK9QAHAiZduoJC3MKd91LPXq1fnKELFzh7Py9WiYoPTHHMOLQgtRUwct5rjc7pzIVRkVESBd2deZ3o6MoNnqOH8mihKUnWGRgCv5UzLL3OS7AswCcshxMl8CHwEW2MYfFoDff%2Bs%2ByajPDJB1Jgrj99XClm%2B4j3inIFuiX0oIBw%2B%2FMYVMTlKllNi5RzBUEItC%2BHOqmaETguzEnljmvnCQ8uzUnln7f4RP3QMrxPkqvt1%2FXHRiTaC3FU%2BXUIpTPZXYciG3d5yFCJbNxtCsJgcAxDbA%2F%2F1U6%2FyaCRD36XfhPLjj0NIPlhyU3u2IShdd2dyU0DeTbAtnf2TW46yLkj0XWuxEjt8oykiTeqovaoHfrCQpxKo10Aqdu4icRIZxaDslgb9Sn%2FivQpdzI0d9RwZEFXP2%2FQ7zz1cmevfQta6lMXFverF62eh9UdGu%2FrssArGHkvDPh1nqL5tI6UR2pDrVU2mv1SMu0ttIoCftWzDoWnpvTOaI2pI4Glt0zLsYrwgignDN9Fyulm5tDM4REI5VFTfyYfIzxPhXtJrLmChscsWyaPZVpRpeolFyloWu81r1tGWU%2Blc3ppTdVVUY4Q8ymWWSjQbxSGeJ3j2d6ZVUa5TOnAyFCEgF6r7hjueVIJk7BGj0n60OMHKTMpkPAUKBgDohsFiTQmZDhO5PHPcmp6ZU4wm0HeP9Y2JaZvolU1uPKJXpl3VHHOYRslgpRKt3msdkrv4Iqktxc4w75jQlcPZGXbxQhwWYNyHQL8vCDXbQ%2Bv7B6142VOlLqBcwUHZjRSaycKgD8cHMOd4jqnOMLSPj3eNW7m80DrWDazHRPzOA4Wi808mRhOOL8zkOaW5HNVR1o07oBuLATfAEvuxjsyMMIkA%2F9oRV%2B%2FFfkawp358xrvY0hUX2xlP9yCtgrkwqNrSBgQJC4SSO8TUUNQZOc5jiv6vaO0aVcl%2FYOVwRVxPeCsqsSmZThVL1lZGyiYYG2U0eREjg2VEpBq3tRyQDM96qli6nw0rBdFjFZTshDjkTFu9XmunmsZBvD5A2vn20Uz76TBoM%2B8nN01hMi53TLFrB6rjI3LEK7WW9lGhNFGKyLX6vRFiF5LtIyYlNAr3oVF13z8nTW5wDrrVNpQa5IxEYivilqmbckRfMog9BxHPKtkhdIHLBJbbbHtsKoKCaNqWk6UPomJvi0ONWNG12TGjANDKE3c08V0X1naK0t7ZWlXwNLG18TSankq52ZpctKzNaxzu5NOavgx7xn5S%2B9lvbxf5bKtEqiapIxHsRTwnKq8N8ZTzbc1uuC91EmjDY5SWjIWIPBPOAQ4mjZs%2BDPtuUgGyyu1nFMkEHc0prvWvsSZbyo%2BVbJwlnt4w1K9RHk0NQlWcqutavmobHPr%2FZe5kyU7maco1OEKJLcW%2B5vl1vEcMsaSWY91L%2Fojh4bSksjk631tnvTKe%2FNzNXSE5i%2BJ9FZeMjNj8Agi7w5xiAOoqXR%2BhIeBl7GXMKcurDXHq3ATnqgI1JXJfq44191OYxWGuyC8ApzzcoYrwDrwu85CAYTprwLHWjwBVUcs5pnPi8zM6%2BlwrGwwayh75VO0oowIAgDld1gy7IbMVOWxgJBYrZe8Xl2WKFGWvhYVTOa4dGmVVCiyNqqqYFBl%2FVMc4zlRJbPqcTadwpmfwx6vdbpMl2ZylcAp8FAg3lMpuDJ3USunZzJnISTItpFsW1G%2BudppAyrblBJwMevJMjCzZlqhpVEaLiTYFJVpRM8GV8dwk3jD8n4XAsSAQ3HoldCV6A0bnnw9IitS6l5xwdAnJG09pkm8iHgdGKw0x8KipFmWsrEJxHM%2BLyv0RFv7G%2FcMBgSV2n%2FJjS0K2yKqJ0Q9KeoFKlcxVae1leXljXmsghkkYcGzoRcoFQnn2iJWpiKJeyU7vCspSSIx8O%2BItNu4qeswSax3ZdE32375I%2FMfPvOmIshVrhSw87G2PpZue8LTtegag0nVg3TjOsPzKhvv05TbFVTdyyxqQk07MJ%2BoKwttg9O2L7cBCqrAHlQbqWC6VMFcSl4hYAtMXNsKxsy8Dt7NMAgaSjlKaaXHZvX%2B9SqqdwuZaI3SHoLV0cJcUFyW8Zk%2Fkyls6nkJ8qNVt5TMthJq14E9JMwH8IUUUzbBE%2F4pP5kTFXcvixaUBmBZFon98IZ9TVf7kOrMGieyGiZR68wLecEwwwzP8Aed8xjpA9q68OC9jOeD3ZRwDljXuJTuUXZA6gOWIfOJBB7avnRhjkKuGoTJQmFrVEFBhc5lbgXLwaDAuiMoaagIG8ql1VCyB65isFYaeHKeJFFO1nJz72TTrnNNfHrkGrl2o8l3YRN2z%2By7tgxfpcKrVHiVCtcqFZpFgHdNIkAdiSxFwHB0OhFQC9A3nnOm4%2FYcR53vYpk6WRXHRL46qmA%2BsGbJmopwsVgv6l6XWfLWKRB%2B9t0Jc72OU2wO17s%2Bf7n99KW18vKZDi1vp7S8la4ijhgaCrUu5dKN82FN6AvAWFyKWgDbA4VGwymtp%2Bzel23cMej2bGvergSO5J%2FKKC1FpWKkiS6cL0Vt%2BF8Fc7Vxgacj1UoHLguN4qdcyf8Io1n5BQ0TSrClKp7qNmBBPjfiU5rMa%2Bd0vKOPs%2FxoTUejQ5NgCJp3dUbQIkVlhG9epEIeQy4zTwwvvX9U0ZsXUU%2BF6tpIye2bZLuQrHCBc3DgGnC95%2Fjjvt%2BOCQ%2B7l4zWSbQgzdQEGU%2Bbf8ks7Z9E5rlm%2FoRn0Sq8gWXqgv2nrt2hT4FtroRa0GtrasJOM6zNjyICs1GaJiQyqF0xNTfpyz6n6zIdNFPtoKkEqW3ottiGJIrukohyEfbuYO6z%2F2O2fJ4mD1i7E8B%2Foq%2Fadf5fK1Jt3g2tt7lnUaomFqI0zz87hCith6aOajT58U3vzu%2B9DWBSaf9GzCDiecVgG92yP5k1B487bR53f6gtLMirnStay2w9%2FsI8Vyd8F7foYmHsXfZrK3MZnLUml9QRoGfjrCPbXHXOWel8vvLV8%2FDVbQeK1Mn0FPvVykjrLoKPb75WmKLOJ62MdPfj52ek7VfiUhipFLEXx0jHsiMlCodnwRnwT8lJx9t1VPoBSMNdojQzjlYr8jkzp%2FTUzRezr60BmJDzFdZIupi%2B8cX2KP%2F9gXcBPjhHKxI986ep3b1hSMpIu2%2FpkLjBv8vuxEm6QpF271GsBLs5dLjjn9rc7OSSG9rtELxV5ptsn96QeAaUxG468ntwJ09RnMHZI%2BLNGPO7j0k6q7aqXpyi8IFDxN0Yk%2BINx3w2vOFE%2FOE7Yl4Y6mCExJwQHpbgY4sSlBufrwnEN1vjTq%2FLdsxlq20TLh1eF%2BP69hD9F62YtImnGfuHi%2Fu6WfW6tq8b7R%2B%2BGMfaaEyPbkifOJt6rXTVl6jXVo3xAPW6KT3mZZbuO7xKFnQSl1AY0WRXt4wH7WhwZ07LIkEqu3ZmbcsCbT1Hm6RIRapCUuQhL1eqBv5RxvCDy2gSRvxkJpF2LD%2FKwanjarFZT09k7mnnv7Fq7fbnOqP0iWzEgc5oSlu9d11n2B9MWFjbdmbytpOS3zFYGrqsOjcsj0H23%2B0OxGzH6moRiLkGT8UeG%2FgIO%2FagEI4yaS%2FNPg6CSR3Jx2YiH83ZaJ%2BvTkNezUty%2BCyezRdbh7rrRmbcScR3Xo7B6j%2BzXMTHd3tmtypooM8I8X0LmtE8b1a5ju%2B2bVRIrowf7h0Rc%2BsRbs8W4e7CX2h3gdVhm%2BTazMhmOxFZ1eXDtN59aYY9D7xBrlv5oFxBXdDPUVjtf2lsdOPDs8YE6Qq8w%2B1DiMbjFY2dj%2FdY2w9W%2BTLMgesLW3q23XMB2oQ78Y3qc2vY0sZpjiYq%2FWOFLd%2Bq%2BmyeUqWl0QvD4jWGeXJJONxCy9slocW0Hx9pL1tDmvVDIN5Ty%2FNzb1tSCJiAgqc3PunCk%2Bdlre2Xo4G1HksxsXf5UjNC3FEL1mpNazoea92uxHXLWk2AoFfWegbW2j4pQdyd1MlzdErO6tp8Lq82xj50XBcwbmtR5Jqi6J9nWXSRx9NVpurxAg3vIRn6bw64NZtdM3duU9K7fbSNERAIbWyrApHwL3ogIk8Le%2FEuv25U7XYTsghcp0%2F52LaYRXl1W%2FTiR5TO8u6jF8GOevtLlaSHVKT4ZkWKrVJTnmx05FiGVa7WNeSt6enP%2B2WzP1ddUU7vvdcbj3tM0XWetd9jeOstM3bc3uiEVs5B4AtGdMWzYOR418Xk1%2BskzQFrDP%2BTuP2WYe9m%2Bwqbj9V4PkFjlIQyDeVOvlnWMOpf%2Fq0qZyqFjhLTIImh8l0UAYrCaYkroKOtbomoc0CBlEofkhoQCKqc%2F%2FuVL%2Fou%2Fr7ly1B6vBrlS0cusIPkS9BevmxL8t%2F9%2BCmT%2FA9ZJeP0DrvU6CjocDypcUdna5oKEI%2Fzc3NLd9okLunnzQv45UZtvsRAsenvmuK%2B1iufgN5LZi1gS7R0pRJC8XMhkLa14ZS4LwptsSfgULN1Es8UcpDqmMLjJiXsqIBPpX%2B9EUjQ4grbXeB7g1Pacx2CNpQIPgowUoDMLAnelGeew8aREI4cAYedS5bQbfGs2pJ3khXJhHw80LpZF9MVnvXjcEr6cbTqx2TZXyQbescbTJzRaOzCc4eJobs0ecyS%2BAiCaAcA5PcjiAZOrfTeJoiCMwqiV%2F9h78U5CtVyu8%2F0V9aqMM94smYOZj3DHPSFOfi9exoP2Wljc6fZlAmbyncAwoVNmfjCkeEEUpo4GIILkT0gVhtaaSXMBTq1wFohMwxiME50tHETIVrBVqNpAgcJmB%2BWAHZUlOUpmRb86l3PBnLDkL3IvLTS6JilrdUwQbeazOY4zmJfcFBkcTSmfiwEpR%2FzklIJYEPzoFqaMHtWJvtJSIuDzr5g3Ylw%2Fi%2Bwc7OsAIuSGRoKJY%2BLd7bS4jeDuuGo1Vzd6QEknwKITtIZzDufOJaHCBO3wDG%2Fri3UFHHMviTeNlMClUikjJN4QwCTx2von%2BgVPz2D7s0NwY%2Bsc%2FdNc9f4Nb%2F2NcbtVgiQ03erC1ZsqUGztnBZGHRjecC3yjP2bcgcpwKhs4p8z2J7Cs%2BkWTG%2Bzbe5%2B%2FHvxrc5qaFU%2BBbBciyoFfsZecdK96qmRnMkVBSGRYpClhRdqYEy4YH%2B0dkEh3CKSb0ooTUAShekNfYXg%2FTp4fnD5JcoxPd%2Fv8MY2wAqDb175xIPAhuQsUagwvdbYrJJufYjIJoKf%2FLtT%2FR%2FPj%2BL48Dh0j2c%2FbDdFV9Thu1sxcJCRLL%2BC467ZOiNmaCRHpQJsNLFLxzp0elKy3Vr9qQyHjWSGQ27UXNbkkydG93KM0HiZIbPuQxdTLo7Gvl9w1PpTlyvXz8J3GZeeEeb9zri1rvy4JLvdeYpf7FhF9rk7%2FFmvp7P%2Bj2LKnc8MbiOOxnXif9YKpB9CerVYfd2T%2FX3twXcicyM0E0K95Q7oA0UUmvLzFiAbkh2NKpzDn9UmzZ5SZ81f3SsWWtRIHuOuRrb5FvQrxOZNG4rNDZ5%2BWxtHm5W45%2F%2Fvfjw9Nn992yz%2Bf1Hd2YxUzUPzW411HOa1NC2OBvMcuVGrfYXt4SV71pH21BWEmPKQ8PbXL1TbaSOvFG5bYJvyJsN%2BBvyEau%2FvnLThsIhH7ADcci7Ozz%2Bjub0dzS%2Fv3zdBsqhhm3gcqgR04dultp0gN%2FEN2azJRm0tWnsrQhLRTtyN08xAHxHUUFlt0hMkSkpSjxlOFKn5onDY3u6j%2FDNnB%2BDiCI2VWAIVVGzHQsmNlP4ymbEqSQkZstaMbL40zoQOHfUaTfZUXERm2BwOa4RHEuhp9fweCyKeBx0SaABAUgxK89KbAxRbAHAaedGaF7VuoOxPYPVFCigKIPhVjUyBRhzFNPOjtI9lM9VfIduBzLLyoW3%2BwPac%2BEmf0%2Fz8UjtgYy2foinN2TyNGbtpByesSZjHmhNZsAQs7zcRnfsDE5QNu%2FURimP8pRJC3oygjxb1TzlknIGccAlYwSQxsYf4acCsBuQQaAfioQWlZQIA4OoeR99H3vAndiK5QLbDvA70HWtO2B7Adhe0qNpE7RJNHxCNyne3LCwGUrDZX9B8mUx7TNKvmfS%2FakPK7hXTHtrxz6Q%2FMdiak37uDxfm0muXZCiN%2FD8vmdoxZbcjWOV0Vopse5ou6NDhyOQTd6wczWsm1j3Q4hLtSDL1nWzMZXq4RdHWajJcFxbqMDiILIUE3RhHlsXqu6Za9zpK0QidvbP7TRJSdZPi3lv6NAN3w%2BTVUcb%2Bi1rmT7wibZt3dX%2FHIIZB6OLI5i6Q3G3Gg%2FrSc0HkYoi8hSXmBsGLP%2Fjn7Omo1GrNR36p1zUuouSL6o8JVCK8p44xegTJLFmhFctgNkHKuHtH7f9IyzmLjl8pqX0%2FLrgtS2lM5HG0QsXk%2F5ME8Ys1b0PDLTxF2pPsyf%2BHw%3D%3D}{https://axa-rev-research.github.io/explaining-fairness-demo.html}
